Loci of 3-periodics in an Elliptic Billiard: why so many ellipses?

A triangle center such as the incenter, barycenter, etc., is specified by a function thrice- and cyclically applied on sidelengths and/or angles. Consider the 1d family of 3-periodics in the elliptic billiard, and the loci of its triangle centers. Some will sweep ellipses, and others higher-degree algebraic curves. We propose two rigorous methods to prove if the locus of a given center is an ellipse: one based on computer algebra, and another based on an algebro-geometric method. We also prove that if the triangle center function is rational on sidelengths, the locus is algebraic

==> 200_biblio.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{DOI~\discretionary{}{}{}#1}\else
  \providecommand{\doi}{DOI~\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi

\bibitem{akopyan2020-invariants}
Akopyan, A., Schwartz, R., Tabachnikov, S.: Billiards in ellipses revisited
  (2020).
\newblock \urlprefix\url{https://arxiv.org/abs/2001.02934}.
\newblock Ar{X}iv

\bibitem{bialy2020-invariants}
Bialy, M., Tabachnikov, S.: {Dan Reznik's} identities and more (2020).
\newblock \urlprefix\url{https://arxiv.org/abs/2001.08469}.
\newblock Ar{X}iv

\bibitem{cox2005-AG}
Cox, D., Little, J., O'Shea, D.: Using Algebraic Geometry.
\newblock Springer (2005)

\bibitem{dragovic11}
Dragovi\'{c}, V., Radnovi\'{c}, M.: Poncelet Porisms and Beyond: Integrable
  Billiards, Hyperelliptic Jacobians and Pencils of Quadrics.
\newblock Frontiers in Mathematics. Springer, Basel (2011).
\newblock \urlprefix\url{https://books.google.com.br/books?id=QcOmDAEACAAJ}

\bibitem{corentin19}
Fierobe, C.: On the circumcenters of triangular orbits in elliptic billiard
  (2018).
\newblock \urlprefix\url{https://arxiv.org/pdf/1807.11903.pdf}.
\newblock Submitted %to {l'Enseign. Math.}

\bibitem{fitzgibbon99-ellipse}
Fitzgibbon, A., Pilu, M., Fisher, R.: Direct least square fitting of ellipses.
\newblock Pattern Analysis and Machine Intelligence \textbf{21}(5) (1999)

\bibitem{ronaldo19}
Garcia, R.: Elliptic billiards and ellipses associated to the 3-periodic
  orbits.
\newblock American Mathematical Monthly \textbf{126}(06), 491--504 (2019).
\newblock \urlprefix\url{https://doi.org/10.1080/00029890.2019.1593087}

\bibitem{griffiths1978}
Griffiths, P., Harris, J.: On {C}ayley's explicit solution to {P}oncelet's
  porism.
\newblock Enseign. Math. (2) \textbf{24}(1-2), 31--40 (1978)

\bibitem{dekov14}
Grozdev, S., Dekov, D.: The computer program “discoverer” as a tool of
  mathematical investigation.
\newblock International Journal of Computer Discovered Mathematics (IJCDM)
  (2014).
\newblock \urlprefix\url{http://www.ddekov.eu/j/2014/JCGM201405.pdf}

\bibitem{kaloshin2018}
Kaloshin, V., Sorrentino, A.: On the integrability of {B}irkhoff billiards.
\newblock Phil. Trans. R. Soc. \textbf{A}(376) (2018).
\newblock \doi{https://doi.org/10.1098/rsta.2017.0419}

\bibitem{kimberling1993_rocky}
Kimberling, C.: Triangle centers as functions.
\newblock Rocky Mountain J. Math. \textbf{23}(4), 1269--1286 (1993).
\newblock \doi{10.1216/rmjm/1181072493}.
\newblock \urlprefix\url{https://doi.org/10.1216/rmjm/1181072493}

\bibitem{etc}
Kimberling, C.: Encyclopedia of triangle centers (2019).
\newblock
  \urlprefix\url{https://faculty.evansville.edu/ck6/encyclopedia/ETC.html}

\bibitem{lang}
Lang, S.: Algebra, \emph{Graduate Texts in Mathematics}, vol. 211, third edn.
\newblock Springer-Verlag, New York (2002).
\newblock \doi{10.1007/978-1-4613-0041-0}.
\newblock \urlprefix\url{https://doi.org/10.1007/978-1-4613-0041-0}

\bibitem{sergei07_grid}
Levi, M., Tabachnikov, S.: The {P}oncelet grid and billiards in ellipses.
\newblock The American Mathematical Monthly \textbf{114}(10), 895--908 (2007).
\newblock \doi{10.1080/00029890.2007.11920482}.
\newblock \urlprefix\url{https://doi.org/10.1080/00029890.2007.11920482}

\bibitem{moore2009-interval-analysis}
Moore, R., Kearfott, R.B., Cloud, M.J.: Introduction to Interval Analysis.
\newblock SIAM (2009)

\bibitem{dsr_applet_x12345}
Reznik, D.: Applet showing the locus of several triangular centers (2019).
\newblock \urlprefix\url{https://editor.p5js.org/dreznik/full/i1Lin7lt7}

\bibitem{dsr_locus_gallery_2019}
Reznik, D.: Triangular orbits in elliptic billards: Loci of points
  {X(1)~X(100)} (2019).
\newblock
  \urlprefix\url{https://dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/loci_6tri.html}

\bibitem{dsr_playlist_2020}
Reznik, D.: Playlist for {``Loci of Triangular Orbits in an Elliptic Billiard:
  Elliptic? Algebraic?''} (2020).
\newblock \urlprefix\url{https://bit.ly/2REOigc}

\bibitem{reznik19}
Reznik, D., Garcia, R., Koiller, J.: Can the elliptic billiard still surprise
  us?
\newblock Mathematical Intelligencer  (2019).
\newblock \doi{10.1007/s00283-019-09951-2}.
\newblock \urlprefix\url{https://arxiv.org/pdf/1911.01515.pdf}

\bibitem{reznik2020-loci}
Reznik, D., Garcia, R., Koiller, J.: Intriguing loci of triangular orbits in
  elliptic billiards (2020).
\newblock In preparation

\bibitem{olga14}
Romaskevich, O.: On the incenters of triangular orbits on elliptic billiards.
\newblock Enseign. Math. \textbf{60}(3-4), 247--255 (2014).
\newblock \doi{10.4171/LEM/60-3/4-2}.
\newblock \urlprefix\url{https://arxiv.org/pdf/1304.7588.pdf}

\bibitem{rozikov2018}
Rozikov, U.A.: An Introduction To Mathematical Billiards.
\newblock World Scientific Publishing Company (2018)

\bibitem{Schenck2003-GA}
Schenck, H.: Computational Algebraic Geometry, London Mathematical Society
  Student Text, vol.~58.
\newblock Cambridge University Press (2003)

\bibitem{snyder92-ellipse}
Snyder, J.M.: Interval analysis for computer graphics.
\newblock Computer Graphics \textbf{26}(2), 121--129 (1992)

\bibitem{Sturmfels97-resultants}
Sturmfels, B.: Introduction to resultants, in Applications of Computational
  Algebraic Geometry, vol.~53, pp. 25--40.
\newblock American Mathematical Society (1997).
\newblock Proceedings of Symposia in Applied Mathematics

\bibitem{sergei91}
Tabachnikov, S.: Geometry and Billiards, \emph{Student Mathematical Library},
  vol.~30.
\newblock American Mathematical Society, Providence, RI (2005).
\newblock \doi{10.1090/stml/030}.
\newblock
  \urlprefix\url{http://www.personal.psu.edu/sot2/books/billiardsgeometry.pdf}.
\newblock Mathematics Advanced Study Semesters, University Park, PA

\bibitem{sergei2016proj}
Tabachnikov, S.: Projective configuration theorems: old wine into new
  wineskins.
\newblock In: S.~Dani, A.~Papadopoulos (eds.) Geometry in History, pp.
  401--434. Springer Verlag (2019).
\newblock \urlprefix\url{https://arxiv.org/pdf/1607.04758.pdf}

\bibitem{mw}
Weisstein, E.: Mathworld (2019).
\newblock \urlprefix\url{http://mathworld.wolfram.com}

\end{thebibliography}

